Secure Software Leasing from Standard Assumptions

Secure software leasing (SSL) is a quantum cryptographic primitive that enables users to execute software only during the software is leased. It prevents users from executing leased software after they return the leased software to its owner. SSL can make software distribution more flexible and controllable. Although SSL is an attractive cryptographic primitive, the existing SSL scheme is based on public key quantum money, which is not instantiated with standard cryptographic assumptions so far. Moreover, the existing SSL scheme only supports a subclass of evasive functions. In this work, we present SSL schemes based on the learning with errors assumption (LWE). Specifically, our contributions consist of the following. - We construct an SSL scheme for pseudorandom functions from the LWE assumption against quantum adversaries. - We construct an SSL scheme for a subclass of evasive functions from the LWE assumption against sub-exponential quantum adversaries. - We construct SSL schemes for the functionalities above with classical communication from the LWE assumption against (sub-exponential) quantum adversaries. SSL with classical communication means that entities exchange only classical information though they run quantum computation locally. Our crucial tool is two-tier quantum lightning, which is introduced in this work and a relaxed version of quantum lighting. In two-tier quantum lightning schemes, we have a public verification algorithm called semi-verification and a private verification algorithm called full-verification. An adversary cannot generate possibly entangled two quantum states whose serial numbers are the same such that one passes the semi-verification, and the other also passes the full-verification. We show that we can construct a two-tier quantum lightning scheme from the LWE assumption.

==> section/proof_relaxed_watermarking_cnc_collusion_resistance.tex <==
% !TEX root = ../main.tex




\begin{proof}[Proof of~\cref{thm:relaxed_watermarking_cnc}]
Let $\qA$ be a QPT adversary attacking relaxed $(1,\Dcnc)$-unremovability.
We prove this theorem using hybrid games.

\begin{description}
\item[Game $1$:]This is $\expa{\qA,\Dcnc}{r}{urmv}(\secp,\epsilon)$ for \cref{const:relaxed_watermarking_cnc}.

\begin{enumerate}
\item The challenger generates $\crs \gets \NIZK.\setup(1^\secp)$ and $\owf\gets\Fow$, and gives $\pp \seteq (\crs,\owf)$ to the adversary $\qA$.
\item At some point, $\qA$ queries messages $(\msg_1,...,\msg_q) \in \M_\secp^q$ to the challenger.
The challenger first samples $\cnc{C}{\alpha}\gets\Dcnc$.
Next, the challenger computes $x \seteq \cS(\cnc{C}{\alpha})$ and $y\gets\owf(\alpha)$.
Then, the challenger computes $\pi_i \gets \NIZK.\Prove(\crs,(\msg_i,\owf,y,C),x)$ for every $i\in[q]$.
Then, the challenger returns $(\tlC_1,...,\tlC_q)$ to $\qA$, where $\tlC_i \seteq (\msg_i,y,C,\pi_i)$.

\item Finally, $\qA$ outputs $\tlC^{\ast}=(\msg^*,y^*,C^*,\pi^*)$. If $\Eval(\pp,\tlC^{\ast},\cdot)$ and $\cnc{C}{\alpha}(\cdot)$ are functionally equivalent, and $\Extract (\pp, \tlC^{\ast}) \ne \msg_i$ for every $i\in[q]$, then the experiment outputs $1$, otherwise $0$.
\end{enumerate}
\end{description}

The output of Game $1$ is $1$ if and only if the following conditions hold in Game $1$.

\begin{itemize}
%\item[$(a)$] $\tlC^{\ast}$ is of the form $(\msg^*,y^*,C^*,\pi^*)$.
\item[$(a)$]  $\Eval(\pp,\tlC^{\ast},\cdot)$ and $\cnc{C}{\alpha}(\cdot)$ are functionally equivalent.
\item[$(b)$] $\NIZK.\vrfy(\crs,(m^*,\owf,y^*,C^*),\pi^*)=\top$.
\item[$(c)$] $\msg^*\neq \msg_i$ for every $i\in[q]$.
\end{itemize}

%We define $\event{S}$ as the event that the above conditions $(a)$,$(c)$,$(d)$, and the following conditions hold.
%\begin{itemize}
%\item[$(b')$]  Let $\omega=\secp/\epsilon^2$. $\Eval(\pp,C^{\ast},x_j)=\PRF.\Eval(\prfkey,x_j)$ holds for some $j\in[\omega]$, where $x_j$ is randomly chosen from the domain of $\PuncPRF$ for every $j\in[\omega]$. 
%\end{itemize}
%We then have $\Pr[\textrm{Output of Game~} 1 \textrm{~is~} 1]\leq \Pr[\event{S}]+\negl(\secp)$.
%This is because when the condition $(b)$ is satisfied, the condition $(b')$ is also satisfied without negligible probability.

We next consider the following adversary $\qAnizk$ attacking true-simulation extractability of $\NIZK$ using $\qA$.

\begin{enumerate}
\item Given $\crs$, $\qAnizk$ generates $\owf\gets\Fow$, and gives $\pp \seteq (\crs,\owf)$ to $\qA$.
\item When $\qA$ queries messages $(\msg_1,...,\msg_q) \in \M_\secp^q$, $\qAnizk$ first samples $\cnc{C}{\alpha}\gets\Dcnc$.
Next, $\qAnizk$ computes $x \seteq \cS(\cnc{C}{\alpha})$ and $y\gets\owf(\alpha)$.
Then, $\qAnizk$ outputs $q$ statement/witness pairs $\{((\msg_i,\owf,y,C),x)\}_{i\in[q]}$.

\item Given $\{\pi\}_{i\in[q]}$, $\qAnizk$ sends $\{\tlC_i\}_{i\in[q]}$ to $\qA$, where $\tlC_i \seteq (\msg_i,y,C,\pi_i)$.

\item When $\qA$ outputs $\tlC^{\ast}=(\msg^*,y^*,C^*,\pi^*)$, $\qAnizk$ first checks whether $\Eval(\pp,C^{\ast},\cdot)$ and $\cnc{C}{\alpha}(\cdot)$ are functionally equivalent.
Note that this check can be done in time $O(2^n)$.
If so, $\qAnizk$ outputs a statement/proof pair $((m^*,\owf,y^*,C^*),\pi^*)$. Otherwise, $\qAnizk$ outputs $\bot$.
\end{enumerate}
$\qAnizk$ perfectly simulates Game $1$ for $\qA$.
\fuyuki{The running time of $\qAnizk$ is bounded by $O(2^\inplen)$.}
When we execute $\expt{\qAnizk,\NIZK}{se\textrm{-}real}$, the output of it is $1$ if and only if the following conditions hold.
\begin{itemize}
\item $\Eval(\pp,\tlC^{\ast},\cdot)$ and $\cnc{C}{\alpha}(\cdot)$ are functionally equivalent.
\item $\NIZK.\vrfy(\crs,(m^*,\owf,y^*,C^*),\pi^*)=\top$.
\item $((\msg_i,\owf,y,C),x)\in \cR_L$ for every $i\in[q]$.
\item $((\msg_i,\owf,y,C),x)\neq(m^*,\owf,y^*,C^*)$ for every $i\in[q]$.
\end{itemize}
We see that when the output of the simulated Game $1$ is 1, the output of $\expt{\qAnizk,\NIZK}{se\textrm{-}real}$ is also $1$.
Namely, we have $\Pr[\textrm{Output of Game~} 1 \textrm{~is~} 1]\leq\Pr[1\gets\expt{\qAnizk,\NIZK}{se\textrm{-}real}]$.

$\qAnizk$ runs in time $O(2^n)$.
Since $\NIZK$ satisfies true-simulation extractability against adversaries runs in time $O(2^n)$, there exist $\fksetup$ and $\Sim=(\Sim_1,\Sim_2)$ such that
\[
\abs{\Pr[1\gets\expt{\qA,\NIZK}{se\textrm{-}real}]-\Pr[1\gets\expt{\qA,\Sim,\NIZK}{se\textrm{-}sim}]}\leq\negl(\secp)
\]
holds.
We define the following Game 2.

\begin{description}
\item[Game $2$:]This game is the same as $\expt{\qAnizk,\Sim,\NIZK}{se\textrm{-}sim}$ except conceptual changes. Especially, this game is obtained by transforming $\expt{\qAnizk,\Sim,\NIZK}{se\textrm{-}sim}$ into a security game played between the challenger and $\qA$ so that the output distribution does not change.
\begin{enumerate}
\item The challenger generates $(\crs,\td)\gets\fksetup(1^\secp)$ and $\owf\gets\Fow$, and gives $\pp \seteq (\crs,\owf)$ to $\qA$.
\item When $\qA$ queries messages $(\msg_1,...,\msg_q) \in \M_\secp^q$, The challenger first samples $\cnc{C}{\alpha}\gets\Dcnc$.
Next, the challenger computes $x \seteq \cS(\cnc{C}{\alpha})$ and $y\gets\owf(\alpha)$.
Then, the challenger computes $(\{\pi_i\}_{i\in[q]},\state_{\Sim})\gets\Sim_1(\crs,\td,\{(\msg_i,\owf,y,C)\}_{i\in[q]})$ and sends $\{\tlC_i\}_{i\in[q]}$ to $\qA$, where $\tlC_i \seteq (\msg_i,y,C,\pi_i)$.

\item When $\qA$ outputs $\tlC^{\ast}=(\msg^*,y^*,\prfkey^*,\pi^*)$, the challenger computes $x^*\gets\Sim_2(\state_{\Sim},(\msg^*,\owf,y^*,C^*),\pi^*)$. The challenger then outputs $1$ if all of the following conditions hold.
\begin{itemize}
\item $\Eval(\pp,C^{\ast},\cdot)$ and $\cnc{C}{\alpha}$ are functionally equivalent.
\item $\NIZK.\vrfy(\crs,(m^*,\owf,y^*,C^*),\pi^*)=\top$.
\item $((\msg_i,\owf,y,C),x)\in \cR_L$ for every $i\in[q]$.
\item $((m^*,\owf,y^*,C^*),x^*)\in \cR_L$.
\item $((\msg_i,\owf,y,C),x)\neq(m^*,\owf,y^*,C^*)$ for every $i\in[q]$.
\end{itemize}
Otherwise, the challenger outputs $0$.
\end{enumerate}
\end{description}

If the above first item and fours item hold, we have
\[
\cnc{C}{\alpha}(x^*)=1 \Leftrightarrow C(x^*)=\alpha,
\]
and thus $\owf(C(x^*))=y$. Therefore, from the security of $\Fow$, we have  $\Pr[\textrm{Output of Game~} 2 \textrm{~is~} 1]\leq\negl(\secp)$.

From the discussions so far, we obtain $\Pr[\textrm{Output of Game~} 1 \textrm{~is~} 1]\leq\negl(\secp)$.
This completes the proof.
\end{proof}

==> section/proof_relaxed_watermarking_prf_collusion_resistance.tex <==
% !TEX root = ../main.tex





\begin{proof}[Proof of~\cref{thm:relaxed_watermarking_prf}]
Let $\qA$ be a QPT adversary attacking relaxed $(\epsilon,\cU_\prfkeyspace)$-unremovability.
We prove this theorem using hybrid games.

\begin{description}
\item[Game $1$:]This is $\expa{\qA,\cU_\prfkeyspace}{r}{urmv}(\secp,\epsilon)$ for \cref{const:relaxed_watermarking_prf}.

\begin{enumerate}
\item The challenger generates $\crs \gets \NIZK.\setup(1^\secp)$ and gives $\pp \seteq \crs$ to the adversary $\qA$.
\item At some point, $\qA$ queries messages $(\msg_1,...,\msg_q) \in \M_\secp^q$ to the challenger.
The challenger first samples $\prfkey \gets\cU_\prfkeyspace$.
Next, the challenger computes $y_{\mv{0}} \gets \PRF.\Eval(\prfkey,\mv{0})$, $\prfkey_{\setbracket{\mv{0}}} \gets \Puncture(\prfkey,\setbracket{\mv{0}})$, and $\pi_i \gets \NIZK.\Prove(\crs,(\msg_i,\prfkey_{\setbracket{\mv{0}}}),\prfkey)$ for every $i\in[q]$.
Then, the challenger returns $(\tlC_1,...,\tlC_q)$ to $\qA$, where $\tlC_i \seteq (\msg_i,y_{\mv{0}},\prfkey_{\setbracket{\mv{0}}},\pi_i)$.

\item Finally, $\qA$ outputs a circuit $C^{\ast}=(\msg^*,y^*,\prfkey^*,\pi^*)$. If it holds that $\Eval(\pp,C^{\ast},\cdot) \cong_{\epsilon} \PRF.\Eval(\prfkey,\cdot)$ and  $\Extract (\pp, C^{\ast}) \ne \msg_i$ for every $i\in[q]$, then the challenger outputs $1$, otherwise $0$.
\end{enumerate}
\end{description}

The output of Game $1$ is $1$ if and only if the following conditions hold in Game $1$.

\begin{itemize}
\item[$(a)$] $\Eval(\pp,C^{\ast},\cdot) \cong_{\epsilon} \PRF.\Eval(\prfkey,\cdot)$.
%\item[$(b)$] $C^{\ast}$ is of the form $(\msg^*,y^*,\prfkey^*,\pi^*)$. 
\item[$(b)$] $\NIZK.\vrfy(\crs,(\msg^*,\prfkey^*),\pi^*)=\top$.
\item[$(c)$] $\msg^*\neq \msg_i$ for every $i\in[q]$.
\end{itemize}
We define $\event{S}$ as the event that the above conditions $(b)$ and $(c)$, and the following condition holds.
\begin{itemize}
\item[$(a')$]  Let $\omega=\secp/\epsilon^2$. $\Eval(\pp,C^{\ast},x_j)=\PRF.\Eval(\prfkey,x_j)$ holds for some $j\in[\omega]$, where $x_j$ is randomly chosen from $\Dprf$ for every $j\in[\omega]$. 
\end{itemize}
%\begin{description}
%\item[$\event{S}$:]In Game 1, the above conditions $(a)$,$(c)$,$(d)$, and the following conditions hold.
%\begin{itemize}
%\item[$(b')$]  Let $\omega=\secp/\epsilon^2$. $\Eval(\pp,C^{\ast},x_j)=\PRF.\Eval(\prfkey,x_j)$ holds for some $j\in[\omega]$, where $x_j$ is randomly chosen from $\calD$ for every $j\in[\omega]$. 
%\end{itemize}
%\end{description}
We then have $\Pr[\textrm{Output of Game~} 1 \textrm{~is~} 1]\leq \Pr[\event{S}]+\negl(\secp)$.
This is because when the condition $(a)$ is satisfied, the condition $(a')$ is also satisfied without negligible probability.

We next consider the following adversary $\qAnizk$ attacking true-simulation extractability of $\NIZK$ using $\qA$.

\begin{enumerate}
\item Given $\crs$, $\qAnizk$ gives $\pp \seteq \crs$ to $\qA$.
\item When $\qA$ queries messages $(\msg_1,...,\msg_q) \in \M_\secp^q$, $\qAnizk$ first samples $\prfkey \gets \cU_\prfkeyspace$.
Next, $\qAnizk$ computes $y_{\mv{0}} \gets \PRF.\Eval(\prfkey,\mv{0})$ and $\prfkey_{\setbracket{\mv{0}}} \gets \Puncture(\prfkey,\setbracket{\mv{0}})$.
Then, $\qAnizk$ outputs $q$ statement/witness pairs $\{((\msg_i,\prfkey_{\setbracket{\mv{0}}}),\prfkey)\}_{i\in[q]}$.

\item Given $\{\pi\}_{i\in[q]}$, $\qAnizk$ sends $\{\tlC_i\}_{i\in[q]}$ to $\qA$, where $\tlC_i \seteq (\msg_i,y_{\mv{0}},\prfkey_{\setbracket{0}},\pi_i)$.

\item When $\qA$ outputs $C^{\ast}=(\msg^*,y^*,\prfkey^*,\pi^*)$, $\qAnizk$ first randomly chooses $x_j$ from $\Dprf$ for every $j\in[\omega]$ and checks whether $\Eval(\pp,C^{\ast},x_j)=\PRF.\Eval(\prfkey,x_j)$ holds for some $j\in[\omega]$.
If so, $\qAnizk$ outputs a statement/proof pair $((m^*,\prfkey^*),\pi^*)$. Otherwise, $\qAnizk$ outputs $\bot$.
\end{enumerate}
$\qAnizk$ perfectly simulates Game $1$ for $\qA$.
When we execute $\expt{\qAnizk,\NIZK}{se\textrm{-}real}$, the output of it is $1$ if and only if the following conditions hold.
\begin{itemize}
\item  Let $\omega=\secp/\epsilon^2$. $\Eval(\pp,C^{\ast},x_j)=\PRF.\Eval(\prfkey,x_j)$ holds for some $j\in[\omega]$, where $x_j$ is randomly chosen from $\Dprf$ for every $j\in[\omega]$. 
\item $\NIZK.\vrfy(\crs,(m^*,\prfkey^*),\pi^*)=\top$.
\item $((\msg_i,\prfkey_{\setbracket{\mv{0}}}),\prfkey)\in \cR_L$ for every $i\in[q]$.
\item $((\msg_i,\prfkey_{\setbracket{\mv{0}}})\neq(m^*,\prfkey^*)$ for every $i\in[q]$.
\end{itemize}
We see that when the event $\event{S}$ occurs in the simulated Game 1, the output of $\expt{\qAnizk,\NIZK}{se\textrm{-}real}$ is $1$.
Namely, we have $\Pr[\event{S}]\leq\Pr[1\gets\expt{\qAnizk,\NIZK}{se\textrm{-}real}]$.

Since $\NIZK$ satisfies true-simulation extractability, there exist $\fksetup$ and $\Sim=(\Sim_1,\Sim_2)$ such that $\abs{\Pr[1\gets\expt{\qA,\NIZK}{se\textrm{-}real}]-\Pr[1\gets\expt{\qA,\Sim,\NIZK}{se\textrm{-}sim}]}\leq\negl(\secp)$ holds.
We define the following Game 2.

\begin{description}
\item[Game $2$:]This game is the same as $\expt{\qAnizk,\Sim,\NIZK}{se\textrm{-}sim}$ except conceptual changes. Especially, this game is obtained by transforming $\expt{\qAnizk,\Sim,\NIZK}{se\textrm{-}sim}$ into a security game played between the challenger and $\qA$ so that the output distribution does not change.
\begin{enumerate}
\item The challenger generates $(\crs,\td)\gets\fksetup(1^\secp)$ and gives $\pp \seteq \crs$ to $\qA$.
\item When $\qA$ queries messages $(\msg_1,...,\msg_q) \in \M_\secp^q$, The challenger first samples $\prfkey \gets \cU_\prfkeyspace$.
Next, the challenger computes $y_{\mv{0}} \gets \PRF.\Eval(\prfkey,\mv{0})$ and $\prfkey_{\setbracket{\mv{0}}} \gets \Puncture(\prfkey,\setbracket{\mv{0}})$.
Then, the challenger computes $(\{\pi_i\}_{i\in[q]},\state_{\Sim})\gets\Sim_1(\crs,\td,\{(\msg_i,\prfkey_{\setbracket{\mv{0}}})\}_{i\in[q]})$ and sends $\{\tlC_i\}_{i\in[q]}$ to $\qA$, where $\tlC_i \seteq (\msg_i,y_{\mv{0}},\prfkey_{\setbracket{0}},\pi_i)$.

\item When $\qA$ outputs $C^{\ast}=(\msg^*,y^*,\prfkey^*,\pi^*)$, the challenger computes $\prfkey'\gets\Sim_2(\state_{\Sim},(\msg^*,\prfkey^*),\pi^*)$.
The challenger then outputs $1$ if all of the following conditions hold.
\begin{itemize}
\item For $\{x_j\}_{j\in[\omega]}$ randomly chosen from $\Dprf$, $\Eval(\pp,C^{\ast},x_j)=\PRF.\Eval(\prfkey,x_j)$ holds for some $j\in[\omega]$.
\item $\NIZK.\vrfy(\crs,x',\pi')=\top$.
\item $((\msg_i,\prfkey_{\setbracket{\mv{0}}}),\prfkey)\in \cR_L$ for every $i\in[q]$.
\item $((\msg^*,\prfkey^*),\prfkey')\in \cR_L$.
\item $(\msg_i,\prfkey_{\setbracket{0}})\neq (\msg^*,\prfkey^*)$ for every $i\in[q]$.
\end{itemize}
Otherwise, the challenger outputs $0$.
\end{enumerate}
\end{description}
When the above first condition and fourth condition hold, we have $\PRF.\Eval(\prfkey,x_j)=\PRF.\Eval(\prfkey',x_j)$.
Then, from the key-injective property of $\PuncPRF$, we also have $\prfkey=\prfkey'$.
Therefore, from the security of$\PuncPRF$, we have $\Pr[\textrm{Output of Game~} 2 \textrm{~is~} 1]\leq\negl(\lambda)$.

From the discussions so far, we obtain $\Pr[\textrm{Output of Game~} 1 \textrm{~is~} 1]\leq\negl(\lambda)$.
This completes the proof.
\end{proof}
